HyperGS: Hyperspectral 3D Gaussian Splatting

We introduce HyperGS, a novel framework for Hyperspectral Novel View Synthesis (HNVS), based on a new latent 3D Gaussian Splatting (3DGS) technique. Our approach enables simultaneous spatial and spectral renderings by encoding material properties from multi-view 3D hyperspectral datasets. HyperGS reconstructs high-fidelity views from arbitrary perspectives with improved accuracy and speed, outperforming currently existing methods. To address the challenges of high-dimensional data, we perform view synthesis in a learned latent space, incorporating a pixel-wise adaptive density function and a pruning technique for increased training stability and efficiency. Additionally, we introduce the first HNVS benchmark, implementing a number of new baselines based on recent SOTA RGB-NVS techniques, alongside the small number of prior works on HNVS. We demonstrate HyperGS's robustness through extensive evaluation of real and simulated hyperspectral scenes with a 14db accuracy improvement upon previously published models.

==> figures/tables/ablation_loss_f.tex <==
\begin{tabular}{lcccc} % 5 columns: 1 for loss function and 4 for metrics
  \toprule
  \multirow{2}{*}{Loss Function} & \multicolumn{4}{c}{Metrics} \\ % Span over the metrics
  \cmidrule(lr){2-5} % Rule between the metrics
           & \PSNR & \SSIM & \MRAE & \RMSE \\
  \midrule
  MSE Loss        & 18.789 & 0.868  & 0.089  & 0.05 \\
  MAE Loss        & 17.124 & 0.823  & 0.107  & 0.06 \\
  Huber Loss      & 18.112 & 0.850  & 0.093  & 0.055 \\
  L1 Loss         & 16.889 & 0.799  & 0.115  & 0.065 \\
  Smooth L1 Loss  & 17.567 & 0.835  & 0.098  & 0.06 \\
  \bottomrule
\end{tabular}

==> figures/tables/ablation_speed.tex <==
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Configuration} & FPS & \begin{tabular}[c]{@{}c@{}}TTR\\ (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Train.T\\  (mins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Eval.T\\  (mins)\end{tabular} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-5} % Separate cmidrules for Configuration and Metrics
Base 3DGS            & 78.1  & 22.22 & 242 & 0.38 \\ 
% \midrule
Decoder in eval only   & 74.2  & 45  & 120 & 0.43 \\
Full decoding in training        & 2.31  & 22.22 & 15 & 1.02 \\
\bottomrule
\end{tabular}


==> figures/tables/average_bayspec.tex <==
% \scriptsize
\begin{tabular}{l cccc | c} 
  \toprule
  \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{Average Results} & \multirow{2}{*}{\FPS} \\  % Adjust the multirow alignment
          & \PSNR & \SSIM & \MRAE & \RMSE & \\
  \cmidrule(lr){1-1} % Rule under the Method column
  \cmidrule(lr){2-5} \cmidrule(lr){6-6}
  
  NeRF         & 23.35 & 0.6061 & 0.0440 & 0.0687 & 0.13 \\
  MipNeRF      & 22.75 & 0.5947 & 0.0435 & 0.0776 & 0.09 \\
  TensoRF   & \yellowc24.66 & \yellowc0.6482 & \yellowc0.0501 & \yellowc0.0587 & 0.17 \\
  Nerfacto     & 19.12 & 0.5866 & 0.0551 & 0.1174 & \yellowc0.50 \\
  MipNerf360     & \orangec26.53 & \orangec0.7442 & \orangec0.0280 & \orangec0.0476 & 0.010 \\
  HS-NeRF      & 19.82 & 0.6714 & 0.0534 & 0.1071 & 0.47 \\
  \midrule
  3DGS         & 22.91 & 0.6321 & 0.1335 & 0.0810 & \redc2.74 \\
  HyperGS    & \redc27.11 & \redc0.7804 & \redc0.0254 & \redc0.0440 & \orangec2.21 \\
  \bottomrule
\end{tabular}


==> figures/tables/average_scannet.tex <==
% \scriptsize
\begin{tabular}{l cccc | c} 
  \toprule
  \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{Average Results} & \multirow{2}{*}{\FPS} \\  % Adjust the multirow alignment
          & \PSNR & \SSIM & \MRAE & \RMSE & \\
  \cmidrule(lr){1-1} % Rule under the Method column
  \cmidrule(lr){2-5} \cmidrule(lr){6-6}
  
  NeRF         & 10.89 & 0.5905 & 0.0625 & 0.3479 & 0.12 \\
  MipNeRF      & 12.53 & 0.5481 & 0.0568 & 0.3198 & 0.091 \\
  TensorF     & 13.00 & 0.5696 & 0.0595 & 0.2780 & 0.092 \\
  Nerfacto     & \yellowc16.37 & \yellowc0.6986 & \yellowc0.0352 & 0.1601 & 0.572 \\
  % MipNeRF360   &  12.28 & 0.6824 & 0.1369 & 0.2658 & \yellowc0.011 \\
  HS-NeRF      & 14.44 & 0.6165 & 0.2037 & \yellowc0.1953 & 0.488 \\
  \midrule
  3DGS         & \orangec28.58 & \orangec0.9627 & \orangec0.0301 & \orangec0.0478 & \redc76.2 \\
  HyperGS    & \redc30.51 & \redc0.9756 & \redc0.00415 & \redc0.0354 & \orangec3.56 \\
  \bottomrule
\end{tabular}


==> figures/tables/average_sop.tex <==
% \scriptsize
\begin{tabular}{l cccc | c} 
  \toprule
  \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{Average Results} & \multirow{2}{*}{\FPS} \\  % Adjust the multirow alignment
          & \PSNR & \SSIM & \MRAE & \RMSE & \\
  \cmidrule(lr){1-1} % Rule under the Method column
  \cmidrule(lr){2-5} \cmidrule(lr){6-6}
  
  NeRF         & 10.89 & 0.5905 & 0.0625 & 0.3479 & 0.12 \\
  MipNeRF      & 12.53 & 0.5481 & 0.0568 & 0.3198 & 0.091 \\
  TensorF     & 13.00 & 0.5696 & 0.0595 & 0.2780 & 0.092 \\
  Nerfacto     & \yellowc16.37 & \yellowc0.6986 & \yellowc0.0352 & 0.1601 & 0.572 \\
  MipNeRF360   &  12.28 & 0.6824 & 0.1369 & 0.2658 & \yellowc0.011 \\
  HS-NeRF      & 14.44 & 0.6165 & 0.2037 & \yellowc0.1953 & 0.488 \\
  \midrule
  3DGS         & \orangec28.58 & \orangec0.9627 & \orangec0.0301 & \orangec0.0478 & \redc3.84 \\
  HyperGS    & \redc30.51 & \redc0.9756 & \redc0.00415 & \redc0.0354 & \orangec3.26 \\
  \bottomrule
\end{tabular}


==> tables/ablation.tex <==
$\displaystyle
\begin{array}{r | ccc | ccc | ccc}\toprule
  \text{Network} & \multicolumn{3}{c}{\text{(BaySpec) Basil}} & \multicolumn{3}{c}{\text{ (SOP) Tools}} & \multicolumn{3}{c}{\text{(scannet) scene0000}} \\
  \text{Architecture} & \text{\PSNR} & \text{\SSIM} & \text{\MRAE}  & \text{\PSNR} & \text{\SSIM} & \text{\MRAE} & \text{\PSNR} & \text{\SSIM} & \text{\MRAE} \\
   \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
  \input{tables/ablation_auto_alt_colorized}
  \\
  \bottomrule
\end{array}
$

==> tables/ablation_auto.tex <==
3DGS      & 13.242 &  0.818 &  0.160     &      16.493 &  0.819 &  0.317     &      15.335 &  0.588 &  0.553 \\
36 Channels      & 12.572 &  0.805 &  0.194     &      16.358 &  0.809 &  0.332     &      14.375 &  0.431 &  0.709 \\
24 Channels      & 12.149 &  0.797 &  0.209     &      16.219 &  0.777 &  0.303     &      15.708 &  0.642 &  0.568 \\
18 Channels   & 11.622 &  0.775 &  0.202     &      16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733 \\
% \bm{C} & \sigma & P_\lambda    & 11.602 &  0.762 &  0.213     &      14.637 &  0.710 &  0.283     &      13.221 &  0.399 &  0.663 \\


==> tables/ablation_auto_alt.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 18.703 &  0.883 &  0.096     &      15.820 &  0.756 &  0.234     &      15.335 &  0.588 &  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      & 18.432 &  0.873 &  0.106     &      15.882 &  0.760 &  0.247     &      14.375 &  0.431 &  0.709 \\
(ours)~\bm{C}_{\phantom{~}} & \sigma_0 & P_0  & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489 \\
\bm{C}_{\phantom{~}} & \sigma & P_0   & 17.477 &  0.863 &  0.090     &      16.532 &  0.792 &  0.237     &       7.958 &  0.333 &  0.621 \\
\bm{C}_2 & \sigma_2 & P_0      & 19.744 &  0.895 &  0.076     &      16.393 &  0.776 &  0.207     &      15.708 &  0.642 &  0.568 \\
\bm{C}_{\phantom{~}} & \sigma & P_\lambda    & 17.494 &  0.851 &  0.128     &      15.265 &  0.704 &  0.312     &      13.221 &  0.399 &  0.663 \\


==> tables/ablation_auto_alt_colorized.tex <==
3DGS      &\cellcolor[rgb]{0.9989300598008057,1,0.9989300598008057} 18.703 &\cellcolor[rgb]{0.9793013022588487,1,0.9793013022588487}  0.883 &\cellcolor[rgb]{0.9961056377100944,1,0.9961056377100944}  0.096     &\cellcolor[rgb]{0.9998852815496433,1,0.9998852815496433}      15.820 &\cellcolor[rgb]{0.9816029333682859,1,0.9816029333682859}  0.756 &\cellcolor[rgb]{0.998559093918138,1,0.998559093918138}  0.234     &\cellcolor[rgb]{0.6805095915200885,1,0.6805095915200885}      15.335 &\cellcolor[rgb]{0.9257498479433259,1,0.9257498479433259}  0.588 &\cellcolor[rgb]{0.9761330572160312,1,0.9761330572160312}  0.553 \\
(Ours) 36 Channels     &\cellcolor[rgb]{0.9999119988152781,1,0.9999119988152781} 18.432 &\cellcolor[rgb]{0.99951171875,1,0.99951171875}  0.873 &\cellcolor[rgb]{0.9999081321873169,1,0.9999081321873169}  0.106     &\cellcolor[rgb]{0.9996692079367389,1,0.9996692079367389}      15.882 &\cellcolor[rgb]{0.9718432426452638,1,0.9718432426452638}  0.760 &\cellcolor[rgb]{0.9997672856233594,1,0.9997672856233594}  0.247     &\cellcolor[rgb]{0.9088677398998146,1,0.9088677398998146}      14.375 &\cellcolor[rgb]{0.9999940930116535,1,0.9999940930116535}  0.431 &\cellcolor[rgb]{0.9999999999576177,1,0.9999999999576177}  0.709 \\
(Ours) 24 Channels  &\cellcolor[rgb]{0.9999725435704786,1,0.9999725435704786} 18.327 &\cellcolor[rgb]{0.9492864884986142,1,0.9492864884986142}  0.886 &\cellcolor[rgb]{0.8822226697131839,1,0.8822226697131839}  0.083     &\cellcolor[rgb]{0.5,1,0.5}      16.548 &\cellcolor[rgb]{1.0,1,1.0}  0.664 &\cellcolor[rgb]{0.5,1,0.5}  0.172     &\cellcolor[rgb]{0.564599133229063,1,0.564599133229063}      15.591 &\cellcolor[rgb]{0.9558160664101377,1,0.9558160664101377}  0.575 &\cellcolor[rgb]{0.5,1,0.5}  0.489 \\
(Ours) 18 Channels   &\cellcolor[rgb]{1.0,1,1.0} 17.477 &\cellcolor[rgb]{0.9999988617027151,1,0.9999988617027151}  0.863 &\cellcolor[rgb]{0.9782843649597519,1,0.9782843649597519}  0.090     &\cellcolor[rgb]{0.5589685202831018,1,0.5589685202831018}      16.532 &\cellcolor[rgb]{0.5,1,0.5}  0.792 &\cellcolor[rgb]{0.9990265754804508,1,0.9990265754804508}  0.237     &\cellcolor[rgb]{1.0,1,1.0}       7.192 &\cellcolor[rgb]{1.0,1,1.0}  0.331 &\cellcolor[rgb]{1.0,1,1.0}  0.733 
% \bm{C}_2 & \sigma_2 & P_0      &\cellcolor[rgb]{0.5,1,0.5} 19.744 &\cellcolor[rgb]{0.5,1,0.5}  0.895 &\cellcolor[rgb]{0.5,1,0.5}  0.076     &\cellcolor[rgb]{0.8620268952777661,1,0.8620268952777661}      16.393 &\cellcolor[rgb]{0.868462211918086,1,0.868462211918086}  0.776 &\cellcolor[rgb]{0.9718432426452637,1,0.9718432426452637}  0.207     &\cellcolor[rgb]{0.5,1,0.5}      15.708 &\cellcolor[rgb]{0.5,1,0.5}  0.642 &\cellcolor[rgb]{0.9900020448758763,1,0.9900020448758763}  0.568 \\
% \bm{C}_{\phantom{~}} & \sigma & P_\lambda    &\cellcolor[rgb]{1.0,1,1.0} 17.494 &\cellcolor[rgb]{1.0,1,1.0}  0.851 &\cellcolor[rgb]{1.0,1,1.0}  0.128     &\cellcolor[rgb]{1.0,1,1.0}      15.265 &\cellcolor[rgb]{0.9999955591079015,1,0.9999955591079015}  0.704 &\cellcolor[rgb]{1.0,1,1.0}  0.312     &\cellcolor[rgb]{0.9841851049096417,1,0.9841851049096417}      13.221 &\cellcolor[rgb]{0.9999998751308253,1,0.9999998751308253}  0.399 &\cellcolor[rgb]{0.9999981117819664,1,0.9999981117819664}  0.663 

==> tables/ablation_auto_bayspec.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 20.279 &  0.734 &  0.295     &      19.084 &  0.705 &  0.530     &      20.102 &  0.729 &  0.399 \\
\bm{C}_1 & \sigma_1 & P_0      & 20.128 &  0.729 &  0.305     &      19.933 &  0.678 &  0.495     &      19.857 &  0.726 &  0.372 \\
(ours)~\bm{C}_{\phantom{~}} & \sigma_0 & P_0  & 20.315 &  0.726 &  0.297     &      19.428 &  0.687 &  0.523     &      20.162 &  0.740 &  0.409 \\
\bm{C}_{\phantom{~}} & \sigma & P_0   & 20.095 &  0.705 &  0.320     &      18.942 &  0.653 &  0.514     &      19.596 &  0.729 &  0.409 \\
\bm{C}_2 & \sigma_2 & P_0      & 21.259 &  0.711 &  0.319     &      18.989 &  0.595 &  0.568     &      19.732 &  0.561 &  0.434 \\
\bm{C}_{\phantom{~}} & \sigma & P_\lambda    & 15.031 &  0.667 &  0.351     &      15.930 &  0.626 &  0.556     &      15.700 &  0.485 &  0.484 \\


==> tables/ablation_auto_bayspec_colorized.tex <==
\text{3DGS (Random Spectra SFM)}                                                           &\cellcolor[rgb]{0.5,1,0.5} 21.259               &\cellcolor[rgb]{0.9827021154333857,1,0.9827021154333857}  0.711 &\cellcolor[rgb]{0.9943158488905341,1,0.9943158488905341}  0.319 &\cellcolor[rgb]{0.9418538319166285,1,0.9418538319166285} 18.989 &\cellcolor[rgb]{1.0,1,1.0}  0.595   
                                                 &\cellcolor[rgb]{1.0,1,1.0}  0.568     &\cellcolor[rgb]{0.7777213941179423,1,0.7777213941179423}      19.732 &\cellcolor[rgb]{0.9999688715641195,1,0.9999688715641195}  0.561 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 \\
\text{(Ours) Base method}      &\cellcolor[rgb]{0.8729040288044295,1,0.8729040288044295} 20.279 &\cellcolor[rgb]{0.5,1,0.5}  0.734 &\cellcolor[rgb]{0.5,1,0.5}  0.295     &\cellcolor[rgb]{0.9257359216835326,1,0.9257359216835326}      19.084 &\cellcolor[rgb]{0.5,1,0.5}  0.705 &\cellcolor[rgb]{0.9973043972155617,1,0.9973043972155617}  0.530     &\cellcolor[rgb]{0.5513230257097693,1,0.5513230257097693}      20.102 &\cellcolor[rgb]{0.6486279830649155,1,0.6486279830649155}  0.729 &\cellcolor[rgb]{0.9449728235767153,1,0.9449728235767153}  0.399 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434\\
\text{(Ours) +Pruning only}      &\cellcolor[rgb]{0.8993767728185065,1,0.8993767728185065} 20.128 &\cellcolor[rgb]{0.731153059388185,1,0.731153059388185}  0.729 &\cellcolor[rgb]{0.8963597524286337,1,0.8963597524286337}  0.305     &\cellcolor[rgb]{0.5,1,0.5}      19.933 &\cellcolor[rgb]{0.9474644525659037,1,0.9474644525659037}  0.678 &\cellcolor[rgb]{0.5,1,0.5}  0.495     &\cellcolor[rgb]{0.7162253002729333,1,0.7162253002729333}      19.857 &\cellcolor[rgb]{0.6817379165683841,1,0.6817379165683841}  0.726 &\cellcolor[rgb]{0.5,1,0.5}  0.372 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434\\
\text{(Ours) +HADC}  &\cellcolor[rgb]{0.8657594741527114,1,0.8657594741527114} 20.315 &\cellcolor[rgb]{0.8192044753625585,1,0.8192044753625585}  0.726 &\cellcolor[rgb]{0.6262201659534103,1,0.6262201659534103}  0.297     &\cellcolor[rgb]{0.8300020341976766,1,0.8300020341976766}      19.428 &\cellcolor[rgb]{0.8802898040092013,1,0.8802898040092013}  0.687 &\cellcolor[rgb]{0.9895747318685465,1,0.9895747318685465}  0.523     &\cellcolor[rgb]{0.5,1,0.5}      20.162 &\cellcolor[rgb]{0.5,1,0.5}  0.740 &\cellcolor[rgb]{0.9797830363557996,1,0.9797830363557996}  0.409 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434
% \text{(Ours) +Lighting}  &\cellcolor[rgb]{0.904471985942854,1,0.904471985942854} 20.095 &\cellcolor[rgb]{0.99464646858295,1,0.99464646858295}  0.705 &\cellcolor[rgb]{0.9955908046679508,1,0.9955908046679508}  0.320     &\cellcolor[rgb]{0.9486281715365203,1,0.9486281715365203}      18.942 &\cellcolor[rgb]{0.9970128813623071,1,0.9970128813623071}  0.653 &\cellcolor[rgb]{0.9551732552758285,1,0.9551732552758285}  0.514     &\cellcolor[rgb]{0.8310784482065837,1,0.8310784482065837}      19.596 &\cellcolor[rgb]{0.6486279830649155,1,0.6486279830649155}  0.729 &\cellcolor[rgb]{0.9797830363557996,1,0.9797830363557996}  0.409 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434 &\cellcolor[rgb]{0.9992111655703528,1,0.9992111655703528}  0.434
% \bm{C}_{\phantom{~}} & \sigma & P_\lambda    &\cellcolor[rgb]{1.0,1,1.0} 15.031 &\cellcolor[rgb]{1.0,1,1.0}  0.667 &\cellcolor[rgb]{1.0,1,1.0}  0.351     &\cellcolor[rgb]{1.0,1,1.0}      15.930 &\cellcolor[rgb]{0.999980106001826,1,0.999980106001826}  0.626 &\cellcolor[rgb]{0.9999997334141514,1,0.9999997334141514}  0.556     &\cellcolor[rgb]{1.0,1,1.0}      15.700 &\cellcolor[rgb]{1.0,1,1.0}  0.485 &\cellcolor[rgb]{1.0,1,1.0}  0.484 


==> tables/ablation_auto_colorized.tex <==
3D GS      &\cellcolor[rgb]{0.5,1,0.5} 13.242 &\cellcolor[rgb]{0.5,1,0.5}  0.818 &\cellcolor[rgb]{0.5,1,0.5}  0.160     &\cellcolor[rgb]{0.5,1,0.5}      16.493 &\cellcolor[rgb]{0.5,1,0.5}  0.819 &\cellcolor[rgb]{0.9999963865521223,1,0.9999963865521223}  0.317     &\cellcolor[rgb]{0.6805095915200885,1,0.6805095915200885}      15.335 &\cellcolor[rgb]{0.9257498479433259,1,0.9257498479433259}  0.588 &\cellcolor[rgb]{0.5,1,0.5}  0.553 \\
(Ours) 36 Channels      &\cellcolor[rgb]{0.9973803162478166,1,0.9973803162478166} 12.572 &\cellcolor[rgb]{0.9643734071913941,1,0.9643734071913941}  0.805 &\cellcolor[rgb]{0.9999824713964786,1,0.9999824713964786}  0.194     &\cellcolor[rgb]{0.7650372650060329,1,0.7650372650060329}      16.358 &\cellcolor[rgb]{0.8089896189767647,1,0.8089896189767647}  0.809 &\cellcolor[rgb]{1.0,1,1.0}  0.332     &\cellcolor[rgb]{0.9088677398998146,1,0.9088677398998146}      14.375 &\cellcolor[rgb]{0.9999940930116535,1,0.9999940930116535}  0.431 &\cellcolor[rgb]{0.9999999991121137,1,0.9999999991121137}  0.709 \\
(Ours) 24 Channels      &\cellcolor[rgb]{0.9999914806828285,1,0.9999914806828285} 12.149 &\cellcolor[rgb]{0.9954525264911352,1,0.9954525264911352}  0.797 &\cellcolor[rgb]{0.9999999999970022,1,0.9999999999970022}  0.209     &\cellcolor[rgb]{0.8987826233403338,1,0.8987826233403338}      16.219 &\cellcolor[rgb]{0.9961500680606966,1,0.9961500680606966}  0.777 &\cellcolor[rgb]{0.9973637342763831,1,0.9973637342763831}  0.303     &\cellcolor[rgb]{0.5,1,0.5}      15.708 &\cellcolor[rgb]{0.5,1,0.5}  0.642 &\cellcolor[rgb]{0.7905480560577024,1,0.7905480560577024}  0.568 \\
(Ours) 18 Channels    &\cellcolor[rgb]{1.0,1,1.0} 11.622 &\cellcolor[rgb]{0.9999997727398665,1,0.9999997727398665}  0.775 &\cellcolor[rgb]{0.9999999258453892,1,0.9999999258453892}  0.202     &\cellcolor[rgb]{0.5,1,0.5}      16.493 &\cellcolor[rgb]{0.9411790890013152,1,0.9411790890013152}  0.798 &\cellcolor[rgb]{0.8295739537151602,1,0.8295739537151602}  0.288     &\cellcolor[rgb]{1.0,1,1.0}       7.192 &\cellcolor[rgb]{1.0,1,1.0}  0.331 &\cellcolor[rgb]{1.0,1,1.0}  0.733 \\
% \bm{C} & \sigma & P_\lambda    &\cellcolor[rgb]{1.0,1,1.0} 11.602 &\cellcolor[rgb]{1.0,1,1.0}  0.762 &\cellcolor[rgb]{1.0,1,1.0}  0.213     &\cellcolor[rgb]{1.0,1,1.0}      14.637 &\cellcolor[rgb]{1.0,1,1.0}  0.710 &\cellcolor[rgb]{0.5,1,0.5}  0.283     &\cellcolor[rgb]{0.9841851049096417,1,0.9841851049096417}      13.221 &\cellcolor[rgb]{0.9999998751308253,1,0.9999998751308253}  0.399 &\cellcolor[rgb]{0.9999604428172743,1,0.9999604428172743}  0.663 \\


==> tables/ablation_bayspec.tex <==
$\displaystyle
\begin{array}{r | cccc c | cccc c | cccc c }\toprule
  \text{Network} & \multicolumn{5}{c}{\text{(BaySpec) Basil}} & \multicolumn{5}{c}{\text{ (SOP) Tools}} & \multicolumn{5}{c}{\text{(scannet) scene0000}} \\
  \text{Architecture} & \text{\PSNR} & \text{\SSIM} & \text{\MRAE} & \text{\FPS} & \text{\train}  & \text{\PSNR} & \text{\SSIM} & \text{\MRAE} & \text{\FPS} & \text{\train} & \text{\PSNR} & \text{\SSIM} & \text{\MRAE} & \text{\FPS} & \text{\train} \\
   \cmidrule(lr){1-1} \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
  \input{tables/ablation_auto_bayspec_colorized}
  \\
  \bottomrule
\end{array}
$

==> tables/old/ablation.tex <==
$$
\begin{array}{ccc | ccc ccc}
  % \rotatebox{-90}{Emittance Network} & \rotatebox{-90}{Transmittance Network} & \rotatebox{-90}{Proposal Network} & \multicolumn{3}{c}{Basil} & \multicolumn{3}{c}{Tools} \\
  \multicolumn{3}{c|}{\text{Network}} & \multicolumn{3}{c}{\text{Basil}} & \multicolumn{3}{c}{\text{Tools}} \\
  \multicolumn{3}{c|}{\text{Archictecure}} & \text{\PSNR} & \text{\SSIM} & \text{\LPIPS} & \text{\PSNR} & \text{\SSIM} & \text{\LPIPS} \\
   \cmidrule(lr){1-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
  %  \text{\hspace*{-6.5em}(HS-NeRF)\hspace*{0.5em}} 
  \input{tables/ablation_auto}
\end{array}
$$

==> tables/old/ablation_auto.tex <==
\bm{C}_1 & \sigma_0 & P_0      & 16.493 &  0.819 &  0.317     &      15.335 &  0.588 &  0.553 \\
\bm{C}_1 & \sigma_1 & P_0      & 16.358 &  0.809 &  0.332     &      14.375 &  0.431 &  0.709 \\
\bm{C}_2 & \sigma_2 & P_0      & 16.219 &  0.777 &  0.303     &      15.708 &  0.642 &  0.568 \\
(ours)~\bm{C} & \sigma & P_0   & 16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733 \\
\bm{C} & \sigma & P_\lambda    & 14.637 &  0.710 &  0.283     &      13.221 &  0.399 &  0.663 \\


==> tables/old/rgb.tex <==
\begin{tabular}[htp]{l ccc ccc ccc ccc} \toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Rosemary} & \multicolumn{3}{c}{Basil} & \multicolumn{3}{c}{Tools} & \multicolumn{3}{c}{Origami} \\
           & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM & \LPIPS & \PSNR & \SSIM & \LPIPS \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
  \input{tables/rgb_auto}
  \bottomrule
\end{tabular}

==> tables/old/rgb_auto.tex <==
nerfacto   & 20.675 &  0.892 &  0.103     &      17.244 &  0.790 &  0.226     &      11.760 &  0.338 &  0.492     &      12.400 &  0.361 &  0.768 \\
Ours-Cont  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &      12.168 &  0.385 &  0.533     &      10.741 &  0.289 &  0.562 \\
Ours-RGB   & 18.601 &  0.865 &  0.083     &      16.780 &  0.765 &  0.212     &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\
Ours-Hyper & 17.702 &  0.870 &  0.094     &      16.493 &  0.798 &  0.288     &       7.192 &  0.331 &  0.733     &      10.359 &  0.453 &  0.693 \\


==> tables/old/rgbauto.tex <==
nerfacto   & 20.675 &  0.892 &  0.103     &      17.244 &  0.790 &  0.226     &      11.760 &  0.338 &  0.492     &      12.400 &  0.361 &  0.768 \\
Ours-Cont  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &        --   &   --   &   --       &      10.741 &  0.289 &  0.562 \\
Ours-RGB   &   --   &   --   &   --       &        --   &   --   &   --       &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\


==> tables/old/wavelength.tex <==
\begin{tabular}[pos]{c ccc ccc cc cc} \toprule
  \# of Wavelengths & \multicolumn{3}{c}{Train Set} & \multicolumn{3}{c}{Unseen Images} & \multicolumn{2}{c}{Unseen Wavelengths} & \multicolumn{2}{c}{Both Unseen} \\
  in Train Set      & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM  & \PSNR & \SSIM  \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
   \input{tables/wavelength_auto}
  \bottomrule
\end{tabular}


==> tables/old/wavelength_auto.tex <==
128        & 20.378 &  0.848 &  0.255 & 16.493 &  0.798 &  0.288 & N/A & N/A & N/A & N/A \\
64         & 19.893 &  0.839 &  0.246 & 16.534 &  0.786 &  0.277 & 20.005 &  0.834 & 16.651 &  0.782 \\
32         & 19.460 &  0.825 &  0.264 & 16.229 &  0.781 &  0.296 & 19.447 &  0.820 & 16.258 &  0.777 \\
16         & 14.592 &  0.759 &  0.272 & 13.586 &  0.717 &  0.306 & 14.656 &  0.759 & 13.641 &  0.717 \\


==> tables/rgb.tex <==
\begin{tabular}[htp]{l ccc ccc ccc ccc} 
  \toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Rosemary} & \multicolumn{3}{c}{Basil} & \multicolumn{3}{c}{Tools} & \multicolumn{3}{c}{Origami} \\
           & \PSNR  & \SSIM & \MRAE & \PSNR  & \SSIM & \MRAE & \PSNR & \SSIM & \MRAE & \PSNR & \SSIM & \MRAE \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
  \input{tables/rgb_auto_colorized}  % This should correctly integrate the rows
  \bottomrule
\end{tabular}


==> tables/rgb_auto.tex <==
NeRF   & 18.789 &  0.868 &  0.089     &      16.147 &  0.714 &  0.229     &      11.760 &  0.338 &  0.492     &      10.371 &  0.220 &  0.560 \\
SpecNeRF  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &      12.168 &  0.385 &  0.533     &      10.741 &  0.289 &  0.562 \\
HS-NeRF   & 18.601 &  0.865 &  0.083     &      16.780 &  0.765 &  0.212     &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\
3DGS & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489     &      10.359 &  0.453 &  0.693 \\
man-splat & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489     &      10.359 &  0.453 &  0.693 \\


==> tables/rgb_auto_bayspec.tex <==
NeRF   & 14.413 &  0.626 &  0.432     &      14.190 &  0.555 &  0.503     &      14.120 &  0.323 &  0.464 \\
SpecNerf  & 14.171 &  0.626 &  0.437     &      14.306 &  0.543 &  0.507     &      13.868 &  0.382 &  0.414 \\
HS-NeRF   & 14.321 &  0.619 &  0.435     &      14.249 &  0.569 &  0.501     &      15.412 &  0.615 &  0.442 \\
3DGS & 20.315 &  0.726 &  0.297     &      19.084 &  0.705 &  0.530     &      20.066 &  0.580 &  0.885 \\
MAN-SPLAT & 25.7 &  0.726 &  0.297     &      19.084 &  0.705 &  0.530     &      20.066 &  0.580 &  0.885 \\

==> tables/rgb_auto_bayspec_colorized.tex <==
NeRF   &\cellcolor[rgb]{0.9999999999999956,1,0.9999999999999956} 14.413 &\cellcolor[rgb]{0.999999999999282,1,0.999999999999282}  0.626 &\cellcolor[rgb]{0.9999999999999983,1,0.9999999999999983}  0.432     &\cellcolor[rgb]{1.0,1,1.0}      14.190 &\cellcolor[rgb]{0.9999999999975132,1,0.9999999999975132}  0.555 &\cellcolor[rgb]{0.7553035510234112,1,0.7553035510234112}  0.503     &\cellcolor[rgb]{0.9999999999999938,1,0.9999999999999938}      14.120 &\cellcolor[rgb]{1.0,1,1.0}  0.323 &\cellcolor[rgb]{0.8372271785727107,1,0.8372271785727107}  0.464 \\
SpecNeRF  &\cellcolor[rgb]{1.0,1,1.0} 14.171 &\cellcolor[rgb]{0.999999999999282,1,0.999999999999282}  0.626 &\cellcolor[rgb]{1.0,1,1.0}  0.437     &\cellcolor[rgb]{1.0,1,1.0}      14.306 &\cellcolor[rgb]{1.0,1,1.0}  0.543 &\cellcolor[rgb]{0.9507656299504499,1,0.9507656299504499}  0.507     &\cellcolor[rgb]{1.0,1,1.0}      13.868 &\cellcolor[rgb]{0.9999999432897442,1,0.9999999432897442}  0.382 &\cellcolor[rgb]{0.5,1,0.5}  0.414 \\
HS-NeRF   &\cellcolor[rgb]{1.0,1,1.0} 14.321 &\cellcolor[rgb]{1.0,1,1.0}  0.619 &\cellcolor[rgb]{1.0,1,1.0}  0.435     &\cellcolor[rgb]{1.0,1,1.0}      14.249 &\cellcolor[rgb]{0.999999994330388,1,0.999999994330388}  0.569 &\cellcolor[rgb]{0.5,1,0.5}  0.501     &\cellcolor[rgb]{0.9999995398205239,1,0.9999995398205239}      15.412 &\cellcolor[rgb]{0.5,1,0.5}  0.615 &\cellcolor[rgb]{0.7291067427204823,1,0.7291067427204823}  0.442 \\
3DGS &\cellcolor[rgb]{0.5,1,0.5} 20.315 &\cellcolor[rgb]{0.5,1,0.5}  0.726 &\cellcolor[rgb]{0.5,1,0.5}  0.297     &\cellcolor[rgb]{0.5,1,0.5}      19.084 &\cellcolor[rgb]{0.5,1,0.5}  0.705 &\cellcolor[rgb]{1.0,1,1.0}  0.530     &\cellcolor[rgb]{0.5,1,0.5}      20.066 &\cellcolor[rgb]{0.8605325940731101,1,0.8605325940731101}  0.580 &\cellcolor[rgb]{1.0,1,1.0}  0.885 \\
MAN-SPLAT &\cellcolor[rgb]{1.0,0.5,0.5} 25.7 &\cellcolor[rgb]{0.5,1,0.5}  0.726 &\cellcolor[rgb]{0.5,1,0.5}  0.297     &\cellcolor[rgb]{0.5,1,0.5}      19.084 &\cellcolor[rgb]{0.5,1,0.5}  0.705 &\cellcolor[rgb]{1.0,1,1.0}  0.530     &\cellcolor[rgb]{0.5,1,0.5}      20.066 &\cellcolor[rgb]{0.8605325940731101,1,0.8605325940731101}  0.580 &\cellcolor[rgb]{1.0,1,1.0}  0.885 \\

==> tables/rgb_auto_colorized.tex <==
NeRF   &\cellcolor[rgb]{0.5,1,0.5} 18.789 &\cellcolor[rgb]{0.9999811099000832,1,0.9999811099000832}  0.868 &\cellcolor[rgb]{1.0,1,1.0}  0.089     &\cellcolor[rgb]{1.0,1,1.0}      16.147 &\cellcolor[rgb]{0.9981963218310892,1,0.9981963218310892}  0.714 &\cellcolor[rgb]{1.0,1,1.0}  0.229     &\cellcolor[rgb]{0.9999999995732687,1,0.9999999995732687}      11.760 &\cellcolor[rgb]{0.9999999997986778,1,0.9999999997986778}  0.338 &\cellcolor[rgb]{0.71580302812135,1,0.71580302812135}  0.492     &\cellcolor[rgb]{0.9999999999999537,1,0.9999999999999537}      10.371 &\cellcolor[rgb]{1.0,1,1.0}  0.220 &\cellcolor[rgb]{0.9389881340995734,1,0.9389881340995734}  0.560 \\
SpecNeRF  &\cellcolor[rgb]{0.999305291675092,1,0.999305291675092} 18.530 &\cellcolor[rgb]{1.0,1,1.0}  0.861 &\cellcolor[rgb]{0.998046875,1,0.998046875}  0.086     &\cellcolor[rgb]{0.999996969646973,1,0.999996969646973}      16.288 &\cellcolor[rgb]{0.9367361182896108,1,0.9367361182896108}  0.742 &\cellcolor[rgb]{0.9999999999988513,1,0.9999999999988513}  0.227     &\cellcolor[rgb]{0.9999996136278253,1,0.9999996136278253}      12.168 &\cellcolor[rgb]{0.9999918765583887,1,0.9999918765583887}  0.385 &\cellcolor[rgb]{1.0,1,1.0}  0.533     &\cellcolor[rgb]{0.9512348340416366,1,0.9512348340416366}      10.741 &\cellcolor[rgb]{0.999970425639529,1,0.999970425639529}  0.289 &\cellcolor[rgb]{0.9459530059631578,1,0.9459530059631578}  0.562 \\
HS-NeRF   &\cellcolor[rgb]{0.9923468768389357,1,0.9923468768389357} 18.601 &\cellcolor[rgb]{0.9999997852516352,1,0.9999997852516352}  0.865 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.5,1,0.5}      16.780 &\cellcolor[rgb]{0.5,1,0.5}  0.765 &\cellcolor[rgb]{0.9999686986888271,1,0.9999686986888271}  0.212     &\cellcolor[rgb]{1.0,1,1.0}      11.456 &\cellcolor[rgb]{1.0,1,1.0}  0.321 &\cellcolor[rgb]{0.9608665245831359,1,0.9608665245831359}  0.501     &\cellcolor[rgb]{0.5,1,0.5}      10.870 &\cellcolor[rgb]{0.999893339703369,1,0.999893339703369}  0.301 &\cellcolor[rgb]{0.5,1,0.5}  0.520 \\
3DGS &\cellcolor[rgb]{1.0,1,1.0} 18.327 &\cellcolor[rgb]{0.5,1,0.5}  0.886 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.9870313340075252,1,0.9870313340075252}      16.548 &\cellcolor[rgb]{1.0,1,1.0}  0.664 &\cellcolor[rgb]{0.5,1,0.5}  0.172     &\cellcolor[rgb]{0.5,1,0.5}      15.591 &\cellcolor[rgb]{0.5,1,0.5}  0.575 &\cellcolor[rgb]{0.5,1,0.5}  0.489     &\cellcolor[rgb]{1.0,1,1.0}      10.359 &\cellcolor[rgb]{0.5,1,0.5}  0.453 &\cellcolor[rgb]{1.0,1,1.0}  0.693 \\
MAN-SPLAT &\cellcolor[rgb]{1.0,1,1.0} 18.327 &\cellcolor[rgb]{0.5,1,0.5}  0.886 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.9870313340075252,1,0.9870313340075252}      16.548 &\cellcolor[rgb]{1.0,1,1.0}  0.664 &\cellcolor[rgb]{0.5,1,0.5}  0.172     &\cellcolor[rgb]{0.5,1,0.5}      15.591 &\cellcolor[rgb]{0.5,1,0.5}  0.575 &\cellcolor[rgb]{0.5,1,0.5}  0.489     &\cellcolor[rgb]{1.0,1,1.0}      10.359 &\cellcolor[rgb]{0.5,1,0.5}  0.453 &\cellcolor[rgb]{1.0,1,1.0}  0.693 \\

==> tables/rgb_bayspec.tex <==
\begin{tabular}[htp]{l ccc ccc ccc} \toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{\textit{Anacampseros}} & \multicolumn{3}{c}{\textit{Caladium}} & \multicolumn{3}{c}{Pinecone} \\
           & \PSNR        & \SSIM & \MRAE & \PSNR           & \SSIM & \MRAE & \PSNR & \SSIM & \MRAE \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-10}
  \input{tables/rgb_auto_bayspec_colorized}
  \bottomrule
\end{tabular}

==> tables/scannet.tex <==
\begin{tabular}[htp]{l ccc ccc ccc ccc} \toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{scene0000} & \multicolumn{3}{c}{scene0000} & \multicolumn{3}{c}{scene0000} & \multicolumn{3}{c}{scene0000} \\
           & \PSNR        & \SSIM & \MRAE & \PSNR           & \SSIM & \MRAE & \PSNR & \SSIM & \MRAE & \PSNR & \SSIM & \MRAE \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
  \input{tables/rgb_auto_colorized}
  \bottomrule
  % \label{tab:scannetSim}
\end{tabular}

==> tables/scannet_auto.tex <==
NeRF   & 18.789 &  0.868 &  0.089     &      16.147 &  0.714 &  0.229     &      11.760 &  0.338 &  0.492     &      10.371 &  0.220 &  0.560 \\
SpecNeRF  & 18.530 &  0.861 &  0.086     &      16.288 &  0.742 &  0.227     &      12.168 &  0.385 &  0.533     &      10.741 &  0.289 &  0.562 \\
HS-NeRF   & 18.601 &  0.865 &  0.083     &      16.780 &  0.765 &  0.212     &      11.456 &  0.321 &  0.501     &      10.870 &  0.301 &  0.520 \\
3DGS & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489     &      10.359 &  0.453 &  0.693 \\
man-splat & 18.327 &  0.886 &  0.083     &      16.548 &  0.664 &  0.172     &      15.591 &  0.575 &  0.489     &      10.359 &  0.453 &  0.693 \\


==> tables/scannet_auto_colour.tex <==
NeRF   &\cellcolor[rgb]{0.5,1,0.5} 18.789 &\cellcolor[rgb]{0.9999811099000832,1,0.9999811099000832}  0.868 &\cellcolor[rgb]{1.0,1,1.0}  0.089     &\cellcolor[rgb]{1.0,1,1.0}      16.147 &\cellcolor[rgb]{0.9981963218310892,1,0.9981963218310892}  0.714 &\cellcolor[rgb]{1.0,1,1.0}  0.229     &\cellcolor[rgb]{0.9999999995732687,1,0.9999999995732687}      11.760 &\cellcolor[rgb]{0.9999999997986778,1,0.9999999997986778}  0.338 &\cellcolor[rgb]{0.71580302812135,1,0.71580302812135}  0.492     &\cellcolor[rgb]{0.9999999999999537,1,0.9999999999999537}      10.371 &\cellcolor[rgb]{1.0,1,1.0}  0.220 &\cellcolor[rgb]{0.9389881340995734,1,0.9389881340995734}  0.560 \\
SpecNeRF  &\cellcolor[rgb]{0.999305291675092,1,0.999305291675092} 18.530 &\cellcolor[rgb]{1.0,1,1.0}  0.861 &\cellcolor[rgb]{0.998046875,1,0.998046875}  0.086     &\cellcolor[rgb]{0.999996969646973,1,0.999996969646973}      16.288 &\cellcolor[rgb]{0.9367361182896108,1,0.9367361182896108}  0.742 &\cellcolor[rgb]{0.9999999999988513,1,0.9999999999988513}  0.227     &\cellcolor[rgb]{0.9999996136278253,1,0.9999996136278253}      12.168 &\cellcolor[rgb]{0.9999918765583887,1,0.9999918765583887}  0.385 &\cellcolor[rgb]{1.0,1,1.0}  0.533     &\cellcolor[rgb]{0.9512348340416366,1,0.9512348340416366}      10.741 &\cellcolor[rgb]{0.999970425639529,1,0.999970425639529}  0.289 &\cellcolor[rgb]{0.9459530059631578,1,0.9459530059631578}  0.562 \\
HS-NeRF   &\cellcolor[rgb]{0.9923468768389357,1,0.9923468768389357} 18.601 &\cellcolor[rgb]{0.9999997852516352,1,0.9999997852516352}  0.865 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.5,1,0.5}      16.780 &\cellcolor[rgb]{0.5,1,0.5}  0.765 &\cellcolor[rgb]{0.9999686986888271,1,0.9999686986888271}  0.212     &\cellcolor[rgb]{1.0,1,1.0}      11.456 &\cellcolor[rgb]{1.0,1,1.0}  0.321 &\cellcolor[rgb]{0.9608665245831359,1,0.9608665245831359}  0.501     &\cellcolor[rgb]{0.5,1,0.5}      10.870 &\cellcolor[rgb]{0.999893339703369,1,0.999893339703369}  0.301 &\cellcolor[rgb]{0.5,1,0.5}  0.520 \\
3DGS &\cellcolor[rgb]{1.0,1,1.0} 18.327 &\cellcolor[rgb]{0.5,1,0.5}  0.886 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.9870313340075252,1,0.9870313340075252}      16.548 &\cellcolor[rgb]{1.0,1,1.0}  0.664 &\cellcolor[rgb]{0.5,1,0.5}  0.172     &\cellcolor[rgb]{0.5,1,0.5}      15.591 &\cellcolor[rgb]{0.5,1,0.5}  0.575 &\cellcolor[rgb]{0.5,1,0.5}  0.489     &\cellcolor[rgb]{1.0,1,1.0}      10.359 &\cellcolor[rgb]{0.5,1,0.5}  0.453 &\cellcolor[rgb]{1.0,1,1.0}  0.693 \\
MAN-SPLAT &\cellcolor[rgb]{1.0,1,1.0} 18.327 &\cellcolor[rgb]{0.5,1,0.5}  0.886 &\cellcolor[rgb]{0.5,1,0.5}  0.083     &\cellcolor[rgb]{0.9870313340075252,1,0.9870313340075252}      16.548 &\cellcolor[rgb]{1.0,1,1.0}  0.664 &\cellcolor[rgb]{0.5,1,0.5}  0.172     &\cellcolor[rgb]{0.5,1,0.5}      15.591 &\cellcolor[rgb]{0.5,1,0.5}  0.575 &\cellcolor[rgb]{0.5,1,0.5}  0.489     &\cellcolor[rgb]{1.0,1,1.0}      10.359 &\cellcolor[rgb]{0.5,1,0.5}  0.453 &\cellcolor[rgb]{1.0,1,1.0}  0.693 \\


==> tables/wavelength.tex <==
\begin{tabular}[pos]{c ccc ccc cc cc} \toprule
  \# of Wavelengths & \multicolumn{3}{c}{Train Set} & \multicolumn{3}{c}{Unseen Images} & \multicolumn{2}{c}{Unseen Wavelengths} & \multicolumn{2}{c}{Both Unseen} \\[0.4em]
  in Train Set      & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM  & \PSNR & \SSIM  \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
   \input{tables/wavelength_auto_colorized}
  \bottomrule
\end{tabular}


==> tables/wavelength_auto.tex <==
128        & 20.378 &  0.848 &  0.255 & 16.493 &  0.798 &  0.288 & N/A & N/A & N/A & N/A \\
64         & 19.893 &  0.839 &  0.246 & 16.534 &  0.786 &  0.277 & 20.005 &  0.834 & 16.651 &  0.782 \\
32         & 19.460 &  0.825 &  0.264 & 16.229 &  0.781 &  0.296 & 19.447 &  0.820 & 16.258 &  0.777 \\
16         & 14.592 &  0.759 &  0.272 & 13.586 &  0.717 &  0.306 & 14.656 &  0.759 & 13.641 &  0.717 \\


==> tables/wavelength_auto_bayspec.tex <==
128        & 20.550 &  0.730 &  0.294 & 20.315 &  0.726 &  0.297 & N/A & N/A & N/A & N/A \\
64         & 20.947 &  0.735 &  0.461 & 20.701 &  0.732 &  0.459 & 20.979 &  0.736 & 20.732 &  0.733 \\
32         & 20.760 &  0.734 &  0.469 & 20.512 &  0.731 &  0.468 & 20.773 &  0.734 & 20.527 &  0.732 \\
16         & 19.868 &  0.727 &  0.477 & 19.705 &  0.725 &  0.474 & 19.854 &  0.728 & 19.690 &  0.726 \\


==> tables/wavelength_auto_bayspec_colorized.tex <==
128        &\cellcolor[rgb]{0.9009277240713697,1,0.9009277240713697} 20.550 &\cellcolor[rgb]{0.9786558295198415,1,0.9786558295198415}  0.730 &\cellcolor[rgb]{0.5,1,0.5}  0.294 &\cellcolor[rgb]{0.9723637950787285,1,0.9723637950787285} 20.315 &\cellcolor[rgb]{0.9999658493272318,1,0.9999658493272318}  0.726 &\cellcolor[rgb]{0.5319894255610764,1,0.5319894255610764}  0.297 & N/A & N/A & N/A & N/A \\
64         &\cellcolor[rgb]{0.5478323939129007,1,0.5478323939129007} 20.947 &\cellcolor[rgb]{0.6584932723174647,1,0.6584932723174647}  0.735 &\cellcolor[rgb]{0.9999707823302408,1,0.9999707823302408}  0.461 &\cellcolor[rgb]{0.8107817780028576,1,0.8107817780028576} 20.701 &\cellcolor[rgb]{0.9180042346834233,1,0.9180042346834233}  0.732 &\cellcolor[rgb]{0.9999531989425561,1,0.9999531989425561}  0.459 &\cellcolor[rgb]{0.5,1,0.5} 20.979 &\cellcolor[rgb]{0.5,1,0.5}  0.736 &\cellcolor[rgb]{0.7864845968605131,1,0.7864845968605131} 20.732 &\cellcolor[rgb]{0.8601188443412335,1,0.8601188443412335}  0.733 \\
32         &\cellcolor[rgb]{0.7625930406799268,1,0.7625930406799268} 20.760 &\cellcolor[rgb]{0.7759374359674885,1,0.7759374359674885}  0.734 &\cellcolor[rgb]{0.99999817389564,1,0.99999817389564}  0.469 &\cellcolor[rgb]{0.917311406449342,1,0.917311406449342} 20.512 &\cellcolor[rgb]{0.9557407280923435,1,0.9557407280923435}  0.731 &\cellcolor[rgb]{0.9999970749339098,1,0.9999970749339098}  0.468 &\cellcolor[rgb]{0.7508435344880633,1,0.7508435344880633} 20.773 &\cellcolor[rgb]{0.7759374359674885,1,0.7759374359674885}  0.734 &\cellcolor[rgb]{0.911108513891689,1,0.911108513891689} 20.527 &\cellcolor[rgb]{0.9180042346834233,1,0.9180042346834233}  0.732 \\
16         &\cellcolor[rgb]{0.9998181813854409,1,0.9998181813854409} 19.868 &\cellcolor[rgb]{0.9994535892357079,1,0.9994535892357079}  0.727 &\cellcolor[rgb]{1.0,1,1.0}  0.477 &\cellcolor[rgb]{0.9999999908309705,1,0.9999999908309705} 19.705 &\cellcolor[rgb]{1.0,1,1.0}  0.725 &\cellcolor[rgb]{0.999999963888073,1,0.999999963888073}  0.474 &\cellcolor[rgb]{0.999868981166906,1,0.999868981166906} 19.854 &\cellcolor[rgb]{0.9972337955057715,1,0.9972337955057715}  0.728 &\cellcolor[rgb]{1.0,1,1.0} 19.690 &\cellcolor[rgb]{0.9999658493272318,1,0.9999658493272318}  0.726 \\


==> tables/wavelength_auto_colorized.tex <==
128        &\cellcolor[rgb]{0.5,1,0.5} 20.378 &\cellcolor[rgb]{0.5,1,0.5}  0.848 &\cellcolor[rgb]{0.9015627978296388,1,0.9015627978296388}  0.255 &\cellcolor[rgb]{0.999896856099743,1,0.999896856099743} 16.493 &\cellcolor[rgb]{0.9959157977845854,1,0.9959157977845854}  0.798 &\cellcolor[rgb]{0.99999704755,1,0.99999704755}  0.288 & N/A & N/A & N/A & N/A \\
64         &\cellcolor[rgb]{0.7616464953959546,1,0.7616464953959546} 19.893 &\cellcolor[rgb]{0.7546108509882288,1,0.7546108509882288}  0.839 &\cellcolor[rgb]{0.5,1,0.5}  0.246 &\cellcolor[rgb]{0.99988134992315,1,0.99988134992315} 16.534 &\cellcolor[rgb]{0.9991782344040058,1,0.9991782344040058}  0.786 &\cellcolor[rgb]{0.9996521135772666,1,0.9996521135772666}  0.277 &\cellcolor[rgb]{0.715771915115113,1,0.715771915115113} 20.005 &\cellcolor[rgb]{0.8385211435321543,1,0.8385211435321543}  0.834 &\cellcolor[rgb]{0.9998248952123672,1,0.9998248952123672} 16.651 &\cellcolor[rgb]{0.9995477374634228,1,0.9995477374634228}  0.782 \\
32         &\cellcolor[rgb]{0.8829604471640253,1,0.8829604471640253} 19.460 &\cellcolor[rgb]{0.9274738535414557,1,0.9274738535414557}  0.825 &\cellcolor[rgb]{0.9858762375500001,1,0.9858762375500001}  0.264 &\cellcolor[rgb]{0.9999601925037106,1,0.9999601925037106} 16.229 &\cellcolor[rgb]{0.9996126917146082,1,0.9996126917146082}  0.781 &\cellcolor[rgb]{0.9999999917309141,1,0.9999999917309141}  0.296 &\cellcolor[rgb]{0.8855250544063498,1,0.8855250544063498} 19.447 &\cellcolor[rgb]{0.9548529586347493,1,0.9548529586347493}  0.820 &\cellcolor[rgb]{0.9999556025762522,1,0.9999556025762522} 16.258 &\cellcolor[rgb]{0.9997968721126531,1,0.9997968721126531}  0.777 \\
16         &\cellcolor[rgb]{0.999999997459185,1,0.999999997459185} 14.592 &\cellcolor[rgb]{0.9999942621399442,1,0.9999942621399442}  0.759 &\cellcolor[rgb]{0.9982929483137318,1,0.9982929483137318}  0.272 &\cellcolor[rgb]{1.0,1,1.0} 13.586 &\cellcolor[rgb]{1.0,1,1.0}  0.717 &\cellcolor[rgb]{1.0,1,1.0}  0.306 &\cellcolor[rgb]{0.9999999952920591,1,0.9999999952920591} 14.656 &\cellcolor[rgb]{0.9999942621399442,1,0.9999942621399442}  0.759 &\cellcolor[rgb]{1.0,1,1.0} 13.641 &\cellcolor[rgb]{1.0,1,1.0}  0.717 \\


==> tables/wavelength_bayspec.tex <==
\begin{tabular}[pos]{c ccc ccc cc cc} \toprule
  \# of Wavelengths & \multicolumn{3}{c}{Train Set} & \multicolumn{3}{c}{Unseen Images} & \multicolumn{2}{c}{Unseen Wavelengths} & \multicolumn{2}{c}{Both Unseen} \\[0.4em]
  in Train Set      & \PSNR        & \SSIM & \LPIPS & \PSNR           & \SSIM & \LPIPS & \PSNR & \SSIM  & \PSNR & \SSIM  \\
  \cmidrule(lr){1-1}      \cmidrule(lr){2-4}              \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
   \input{tables/wavelength_auto_bayspec_colorized}
  \bottomrule
\end{tabular}

